HardTaint: Production-Run Dynamic Taint Analysis via Selective Hardware Tracing

Dynamic taint analysis (DTA), as a fundamental analysis technique, is widely used in security, privacy, and diagnosis, etc. As DTA demands to collect and analyze massive taint data online, it suffers extremely high runtime overhead. Over the past decades, numerous attempts have been made to lower the overhead of DTA. Unfortunately, the reductions they achieved are marginal, causing DTA only applicable to the debugging/testing scenarios. In this paper, we propose and implement HardTaint, a system that can realize production-run dynamic taint tracking. HardTaint adopts a hybrid and systematic design which combines static analysis, selective hardware tracing and parallel graph processing techniques. The comprehensive evaluations demonstrate that HardTaint introduces only around 9% runtime overhead which is an order of magnitude lower than the state-of-the-arts, while without sacrificing any taint detection capability.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> impact.tex <==
\MyPara{Comparisons with Software-based Approach and Naive Hardware Tracing.}
To demonstrate the necessity of runtime selective tracing, we evaluate the runtime overhead, statistics of instruction counts, and data loss of HardTaint, the representative software-based approach (\ie, SelectiveTaint \cite{chen2021selectivetaint}), and naive hardware tracing (NHT for short).
To be precise, as the most recent software-based approach, SelectiveTaint \cite{chen2021selectivetaint} follows the traditional DTA mechanism to perform dynamic taint tracking via software instrumentation. 
%\zyy{It leverages static analysis to remove unnecessary taint tracking to some extent.} 
It has neither fine-grained identification analysis to prune away unnecessary registers nor hardware tracing. 
For NHT, the whole-program control-flow information are traced via Intel PT by default. All the registers needed are recorded via \emph{ptwrite} instructions. NHT has the advantage of hardware tracing, while without the selective tracing capability (\ie, static identification analysis + selective binary writing).


%\MyPara{Identification Analysis.}
TO indicates the time overhead in Table \ref{tab:compare-to-st-naively-tracing}.
Column $S_{inst}$  shows the number of instructions identified by static analysis, along with the proportion relative to the total number of instructions in each binary. \textbf{$D_{inst}$} denotes the exact number of instructions to be traced dynamically.
%This further demonstrates the excellent scalability and applicability of HardTaint.
%Furthermore, the results of dynamic execution also corroborate the advantages of our identification analysis.
Due to the severe data loss in NHT, we cannot accurately count the exact number of dynamically traced instructions.
Instead, we collect the number of times data loss happened during tracing denoted by LT and  the effect of lost data on taint propagation represented by EF, where \pie{0}, \pie{90}, \pie{180} and \pie{360} denote no effect, taint-related memory address loss, memory address recovery failure, and control-flow recovery failure, respectively.
Note that SelectiveTaint failed to instrument the binaries, \emph{gcc}, \emph{xalan}, \emph{PHP}, and \emph{MySQL}. 
OOT means SelectiveTaint failed to complete the static analysis within 120 hours, showing that the static analysis proposed by SelectiveTaint is of poor scalability. 
\zyy{Further, Table \ref{tab:compare-with-selectivetaint-static} provides a detailed comparison of the static analysis time of HardTaint and SelectiveTaint. It shows that HardTaint's analysis time is significantly shorter than SelectiveTaint, especially on \emph{gcc} and \emph{xalan}. On average, HardTaint's analysis performance is 24.25x faster than SelectiveTaint.}

\begin{table}[htb!]
\caption{Static analysis time in seconds of HardTaint and SelectiveTaint.}
\label{tab:compare-with-selectivetaint-static}
\scalebox{0.76}{
\begin{tabular}{c|c|c|c}
\hline
Subject    & SelectiveTaint (sec.) & HardTaint (sec.) & SpeedUp \\ \hline
\hline
coreutils  & 48             & 16        & 3.00x    \\ \hline
gzip       & 50             & 18        & 2.78x    \\ \hline
scp        & 8              & 9         & 0.89x    \\ \hline
tar        & 825            & 118       & 6.99x    \\ \hline \hline
exim       & 3,608           & 480       & 7.52x    \\ \hline
memcached  & 83             & 25        & 3.32x    \\ \hline
nginx      & 2,973           & 461       & 6.45x    \\ \hline \hline
astar      & 20             & 16        & 1.25x    \\ \hline
bzip2      & 38             & 44        & 0.86x    \\ \hline
gcc        & 129,628              & 5,066        & 25.59x    \\ \hline
gobmk      & 6,154           & 517       & 11.90x   \\ \hline
h264ref    & 1,901           & 588       & 3.23x    \\ \hline
hmmer      & 640            & 116       & 5.52x    \\ \hline
libquantum & 24             & 13        & 1.85x    \\ \hline
mcf        & 3              & 8         & 0.38x    \\ \hline
omnetpp    & 3,258           & 773       & 4.21x    \\ \hline
perlbench  & 8,691           & 968       & 8.98x    \\ \hline
sjeng      & 104            & 27        & 3.85x    \\ \hline
xalan        & 216,172              & 6,166        & 35.08x    \\ \hline
\hline
Average        &      19,696   & 812    & 24.25x    \\ \hline
\end{tabular}
}
\end{table}

%Since this number depends on the input size and the subject itself, it can vary widely.
%To facilitate comparison, we use the ratio $D_{ST} / D_{HT}$, representing the number of dynamically traced instructions of SelectiveTaint divided by HardTaint's.
%Consequently, the ratios are all significantly greater than 1, indicating that SelectiveTaint dynamically traced much more instructions than HardTaint.
%Although the ratios are not that large, the significant base of instruction counts makes even a slight difference result in a substantial impact on performance.
% \zyy{todo...}For the runtime overhead, comparing NTWOI and NTWI, it is found that with identification analysis enabled, NTWI lowers the average overhead from 79.69\% (NTWOI) to 23.92\%. 

%\MyPara{Selective Tracing.}
As can be seen \zyy{in Table \ref{tab:compare-to-st-naively-tracing}},  the runtime overhead of software-based approach (\ie, SelectiveTaint) is significantly (orders-of-magnitude) higher than that of HardTaint. This is because SelectiveTaint has to maintain the large amount of taint information, and perform the heavy taint operations (such as looking up and updating taint information) at runtime.
%Thus, each taint operation such as looking up and updating for taint information is heavy.
This accumulates and eventually leads to the prohibitively high overhead.
% \zyy{In contrast, as the input scale grows, a portion of the inherent trace overhead is amortized over the running time, resulting in a decrease in the percentage of overhead for HardTaint.}

In contrast, thanks to the fine-grained identification analysis, the number of traced instructions in \tool is much smaller than that in the representative software-based approach (\ie, SelectiveTaint).
\zyy{In terms of the number of instructions to be traced statically (\ie, $S_{inst}$), SelectiveTaint traces an average of 70.37\% of instructions, while HardTaint only traces 11.00\%. In other words, SelectiveTaint eliminates 29.63\% (100\%-70.37\%) of instructions that are irrelevant to taint analysis, while HardTaint's identification analysis further prunes away 59.37\% (70.37\%-11.00\%) of redundant instructions.
Comparing the dynamic number $D_{inst}$ — the number of instructions recorded dynamically (given that one instruction can be executed multiple times) — HardTaint traces significantly fewer instructions at runtime than SelectiveTaint (\ie, $5.19 \times 10^8$ vs. $10.15 \times 10^8$).
Besides, HardTaint's identification analysis further contributes to the performance. By comparing HardTaint and NHT (which leverages hardware tracing but does not apply identification analysis), as shown in Table \ref{tab:compare-to-st-naively-tracing}, there is a notable reduction in runtime overhead, from an average of 79.69\% down to 9.06\%.
}
In a word, \zyy{our static identification analysis provides significant contributions}, and \tool only records a small portion of necessary taint data via selective hardware tracing and does not perform any operations of taint analysis at runtime.

For naive hardware tracing, although it achieves  the significant performance improvement over software-based approach ($\sim$547.42\% for SelectiveTaint), its overhead  ($\sim$79.69\% on average) is still high and inadequate to meet production-run requirements. 
Even worse, NHT suffers from frequent and severe data loss, leading to catastrophic effects on taint propagation (shown as Columns LT and EF).
% Even with the adoption of identification analysis (\ie, NTWI), although the runtime overhead has been substantially reduced from 79.69\% to 23.92\% and data loss has been improved to some extent, it still falls short of meeting the requirements for precise taint analysis.
In contrast, \tool reduces the overhead to 9.06\% thanks to runtime selective tracing. More importantly, it has no data loss on any subject, offering completely precise taint analysis as the software-based approaches.
The reason is because \tool only needs to generate the PTW and FUP packets for the branch targets and registers of interest.
While the naive hardware tracing has to record all the branches generating a massive amount of non-informative data (\eg, PGE and PGD), as well as a great number of redundant register values.

